A unified formulation of splitting-based implicit time integration schemes

Splitting-based time integration approaches such as fractional steps, alternating direction implicit, operator splitting, and locally one-dimensional methods partition the system of interest into components and solve individual components implicitly in a cost-effective way. This work proposes a unified formulation of splitting time integration schemes in the framework of general-structure additive Runge-Kutta (GARK) methods. Specifically, we develop implicit-implicit (IMIM) GARK schemes, provide the order conditions and stability analysis for this class, and explain their application to partitioned systems of ordinary differential equations. We show that classical splitting methods belong to the IMIM GARK family, and therefore can be studied in this unified framework. New IMIM-GARK splitting methods are developed and tested using parabolic systems.

==> Include/linear_invariants.tex <==
%%%%%%%%%%%%%%%%%%%%%
\section{Linear invariants}
%%%%%%%%%%%%%%%%%%%%%

Consider a linear invariant of the overall system:
\begin{equation*}
	\zeta^\tp \cdot \sum_{m=1}^{\nparts} f\comp{m}(t,y) = 0
	\quad \Rightarrow \quad
	\zeta^\tp\cdot y(t) = \textnormal{const}.
\end{equation*}
%
Clearly, if each process preserves the linear invariant, $\zeta^\tp\cdot f\comp{m}(t,y) = 0$ $\forall m$, then the GARK solution preserves it at well.

The difficulty in general is that each process has a different argument. The invariant relation implies that
%
\[
\sum_\ell  \zeta^\tp\cdot f\comp{\ell}(T_j,Y_j\comp{p}) = 0 \quad\textnormal(for~ fixed~ p).
\]
%
The total is zero when all the functions are evaluated at the same argument. However, when each function has its own argument
%
\[
\sum_\ell  \zeta^\tp\cdot f\comp{\ell}(T_j,Y_j\comp{\ell}) \ne 0.
\]
%
Let $\phi_j\comp{p} = \zeta^\tp \cdot f\comp{p}(T_j,Y_j\comp{p})$ and $\mu_j\comp{p} = \zeta^\tp \cdot Y_j\comp{p}$. Multiply the Kronecker-form \cref{eqn:GARK-Kronecker-form} by $\zeta^\tp$ from the left, to obtain:
%
\begin{equation} 
\label{eqn:conservation-Kronecker-form}
\begin{split}
\mu &= \one{\nparts}\, m_n + \Dt\,\Atilde \, \phi, \\
m_{n+1} &= m_n + \Dt\,\btilde\,^\tp\, \phi = 
\begin{cases}
m_n + \btilde\,^\tp\, \Atilde \,^{-1}\, (\mu - \one{\nparts}\, m_n) & \Atilde~\textrm{nonsingular} \\
m_n + e_s\,^\tp\,(\mu - \one{\nparts}\, m_n) & \textrm{stiffly accurate} 
\end{cases}
\end{split}
\end{equation}


%\begin{equation}
%\begin{split}
%\texttt{for}~~i = 1,\dots, s: &\\
%\nonumber
%\texttt{for}~p=1,\dots,\nparts: &\\
%\mu_i\comp{p}  &= \mu_{n} 
% + \Dt \sum_{j=1}^{i}  a_{i,j}^{\I} \, \left( \sum_{\ell=1}^p \phi\comp{\ell}_j  \right) 
% + \Dt \sum_{j=1}^{i-1}  a_{i,j}^{\E} \, \left( \sum_{\ell=p+1}^\nparts \phi\comp{\ell}_j \right); \\
%\nonumber
%\texttt{end}~\texttt{for}~p &\\
%\nonumber
%\texttt{end}~\texttt{for}~i &\\
%\mu_{n+1} &= \mu_n  + \Dt\sum_{i=1}^{s} b_{i} \, 
% \left( \sum_{\ell=1}^\nparts \phi\comp{\ell}_i   \right)\,.
% \end{split}
%\end{equation}


